Comprehensive Robotic Cholecystectomy Dataset (CRCD): Integrating Kinematics, Pedal Signals, and Endoscopic Videos

In recent years, the potential applications of machine learning to Minimally Invasive Surgery (MIS) have spurred interest in data sets that can be used to develop data-driven tools. This paper introduces a novel dataset recorded during ex vivo pseudo-cholecystectomy procedures on pig livers, utilizing the da Vinci Research Kit (dVRK). Unlike current datasets, ours bridges a critical gap by offering not only full kinematic data but also capturing all pedal inputs used during the procedure and providing a time-stamped record of the endoscope's movements. Contributed by seven surgeons, this data set introduces a new dimension to surgical robotics research, allowing the creation of advanced models for automating console functionalities. Our work addresses the existing limitation of incomplete recordings and imprecise kinematic data, common in other datasets. By introducing two models, dedicated to predicting clutch usage and camera activation, we highlight the dataset's potential for advancing automation in surgical robotics. The comparison of methodologies and time windows provides insights into the models' boundaries and limitations.

==> classifiers.tex <==
\section{Classifiers}

\subsection{Support Vector Machine}
Support Vector Machine (SVM)~\cite{cortes1995support} is a linear predictor that can train and classify nonlinear data points by first mapping the data set to a high-dimensional space using kernels. SVM then searches for a hyperplane that can separate the mapped training set with the largest possible margin into two binary classes. 

\subsection{Ensemble Learning with Decision Trees}
The random forest algorithm~\cite{breiman2001random} generates a bootstrap sample from the entire training set and uses it to train a classification and regression tree (CART)~\cite{breiman2017classification} based on the values in an independent and identically distributed random vector. During testing, the output is determined by selecting the class with the highest number of votes from the predictions of the trees for the given input.

\subsubsection{Adaptive Boosting}
We explored another popular ensemble method known as Adaptive Boosting (AdaBoost) for multiclass classification~\cite{freund1997decision}. AdaBoost first distributes equal weights to all training samples and then trains a decision stump (decision trees with one split). The weights of misclassified observations increase while the weights of correctly classified ones decrease. It repeats the process for certain iterations and a more complicated error metric known as pseudo-loss~\cite{freund1997decision} is used. The prediction method is similar to random forests except that the votes are weighted for each learner based on the pseudo-loss.

\subsubsection{Light Gradient Boosting Machine (L-GBM) Classifier}
In L-GBM ~\cite{NIPS2017_6449f44a}, decision trees are added sequentially, with each tree correcting errors made by the ensemble of previous trees. Unlike traditional gradient boosting methods, L-GBM focuses on minimizing the loss function directly. It is designed for distributed and efficient training of large datasets, making it suitable for applications with resource constraints. L-GBM is known for its leaf-wise growth strategy, efficient handling of categorical features, and parallel/distributed training capabilities. 


\subsection{Feedforward Neural Networks}
Feedforward neural networks (FNNs), also known as multilayer perceptrons (MLPs), are a classic method for classifying nonlinear data~\cite{Goodfellow-et-al-2016}. In this study, we trained a neural network with a specific structure, consisting of an input layer ($n_{0}$) sized according to the number of features, followed by two fully connected layers ($n_{1}, n_{2}$) where the number of neurons in each layer is proportional to the previous layer's size ($n_{1}=\alpha_1 n_{0}, n_{2}=\alpha_2 n_{1}, 2/3 \leq \alpha_1, \alpha_2 \leq 2$). Specific values of the $\alpha_1$ and $\alpha_2$ were determined with Bayesian hyper-parameter optimization method~\cite{snoek2012practical}. The motivation for choosing this specific layer structure was to balance the data-to-model size ratio. With the above conservative structure of the network, the total number of training weights grows quadratically as a function of the number of input neurons:
\begin{equation}
    % N = n_{0}^2 (\alpha+\alpha^3) + \alpha^2 n_{0}n_{f}
    N = n_{0}^2 (\alpha_1+\alpha_1^2\alpha_2) + \alpha_1\alpha_2 n_{0}n_{f}
\end{equation}
The final layer ($n_{f}$) has $N+1$ outputs that correspond to the number of classes. We used the rectified linear unit (ReLU) as the activation function for the first two layers and the Softmax function for the final layer. To minimize the cross-entropy loss, the limited-memory Broyden-Fletcher-Goldfarb-Shanno quasi-Newton algorithm (LBFGS) was employed~\cite{nocedal2006numerical}.



==> tables/table_calibration.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|l}
\hline
\hline
\textbf{Measure (distance)}          & \textbf{dVRK $\Leftrightarrow$ ArUco }     & \textbf{Custom $\Leftrightarrow$ ArUco} \\ \hline

\multirow{3}{*}{Mean Error}          &X: $11.0mm$                                &X: $5.6mm$                               \\
                                     &Y: $50.1mm$                                &Y: $2.5mm$                               \\
                                     &Z: $20.9mm$                                &Z: $1.1mm$                               \\ \hline
\multirow{3}{*}{Standard deviation}  &X: $4.9mm$                                &X: $3.6mm$                               \\
                                     &Y: $2.0mm$                                &Y: $2.1mm$                               \\
                                     &Z: $3.9mm$                                &Z: $2.2mm$                               \\
\hline
\hline
\end{tabular}%
}
\caption{The first Row shows the distance between the kinematics data obtained by dVRK compared to the one obtained by detecting the ArUco markers, while the second row shows the distance between the kinematics data by our custom calibration compared to the one obtained by detecting the ArUco markers. We can observe that the mean error decreases drastically (a factor of 1.96 for X, 20.04 for Y, and 19 for Z). }
\label{tab:calib_table}
\vspace{-7mm}
\end{table}
